X-Learner: Learning Cross Sources and Tasks for Universal Visual Representation

In computer vision, pre-training models based on largescale supervised learning have been proven effective over the past few years. However, existing works mostly focus on learning from individual task with single data source (e.g., ImageNet for classification or COCO for detection). This restricted form limits their generalizability and usability due to the lack of vast semantic information from various tasks and data sources. Here, we demonstrate that jointly learning from heterogeneous tasks and multiple data sources contributes to universal visual representation, leading to better transferring results of various downstream tasks. Thus, learning how to bridge the gaps among different tasks and data sources is the key, but it still remains an open question. In this work, we propose a representation learning framework called X-Learner, which learns the universal feature of multiple vision tasks supervised by various sources, with expansion and squeeze stage: 1) Expansion Stage: X-Learner learns the task-specific feature to alleviate task interference and enrich the representation by reconciliation layer. 2) Squeeze Stage: X-Learner condenses the model to a reasonable size and learns the universal and generalizable representation for various tasks transferring. Extensive experiments demonstrate that X-Learner achieves strong performance on different tasks without extra annotations, modalities and computational costs compared to existing representation learning methods. Notably, a single X-Learner model shows remarkable gains of 3.0%, 3.3% and 1.8% over current pretrained models on 12 downstream datasets for classification, object detection and semantic segmentation.

==> content/0.abstract_bak.tex <==

\begin{abstract}

Visual representation learning from large-scale supervised pre-training has achieved substantial progress. However, existing works tend to focus on individual task (e.g. either classification or detection) and individual data source (e.g. either ImageNet or COCO) separately.
% , leading to suboptimal representation learning. 
The vast semantic information available from different tasks and data sources is largely ignored.
%
Here we argue that jointly learning across heterogeneous tasks and diverse sources induces universal visual representation, which transfers well to various downstream benchmarks.
Nonetheless, how to effectively bridge the gaps among different tasks and sources remains an open question.
In this work, we propose a new pre-training paradigm, \textbf{\framework{}}, which leverages cross-task and cross-source information in a unified framework, with two dedicated stages:
% \textcolor{red}{It first learns the specific representation within homogenise tasks of multiple domains, relieving task conflict issue. Then we do knowledge integration by information and capacity expansion. Finally, we squeeze the model back to a reasonable complexity, but preserving the robust representation.}
\textbf{1) \dilationstage{}:} X-Learner first integrates knowledge across heterogeneous tasks of multiple sources by a capacity expansion, which effectively alleviates task interference. 
\textbf{2) \squeezestage{}:} X-Learner then produces a unified and generalizable representation while squeezing model complexity to a reasonable level.
%
% \textcolor{red}{Moreover, we perform in-depth analysis of the effect of joint training diverse tasks by carrying out an experimental exploration of transfer learning across vastly different data domains, task types and methods. And our study leads to several insights and recommendations for this new diagram.} 
% \textcolor{blue}{Moreover, we perform in-depth analysis of the effect of joint training diverse tasks by carrying out an experimental exploration of transfer learning across heterogeneous tasks, diverse data, and proposed dilation layer and squeeze layer. Our study leads to several insights and recommendations for this new diagram.}
Moreover, we perform an in-depth analysis of this multi-task, multi-source pre-training paradigm as well as effects of the two stages.
% the dilation stage and the squeeze stage.
%
Extensive experiments demonstrate that X-Learner has superior representation learning and generalization ability compared to other pre-training alternatives.
Notably, a single X-Learner model shows remarkable gains of 3.0\%, 3.3\% and 1.8\% over the ImageNet pre-trained model on 12 downstream datasets for classification, object detection and semantic segmentation.
% , validating the effectiveness of X-Learner for universal visual representation.
\end{abstract}

% % 从获取 general representation 入手，给人的第一印象应该是 general representation，而不是 MTL 这个方法；
% We are interested in learning a single general model that transfer well for tasks of various categories.
% % 目前representation比较limited，特定方向的预训练，没有融合起来
% Most current representation learning approaches are optimized for either specialized task, or oversimplified by design and may miss the peculiarity needed in tasks. The complex circumstances in which these representations expected to consistently work are not well discussed.
% % 然后引入 MTL，说明 MTL as pretraining 这个事情还没有得到重视或者探索，原因可能有哪些；
% Traditional multi-task learning approaches learn the common knowledge between a collection of related tasks. However, a more potential usage, yet under-explored, is for pretraining.
% % % task conflict by 异构任务
% We argue one reason is that choosing which tasks should be learned jointly is a non-trivial problem. 
% % single-dataset 限制，non-trivial
% And most works rely on a single dataset with multi-task annotations, which is limited by domains and hard to scale up.
% % 强调我们是第一个充分 study 或者 investigate 了 MTL as pretraining 这件事情的工作，说明我们是一种在 supervised learning 上延生出去的新预训练范式，以及包括哪些特点和优点；
% We introduce a new pretraining paradigm, named X-Learner, from the perspective of multi-task learning. It first learns the specific representation within homogenise tasks of multiple domains, relieving task conflict issue. Then we do knowledge integration by information and capacity expansion. Finally, we squeeze the model back to a reasonable complexity, but preserving the robust representation. The X-Learner can effectively exploit the knowledge cross tasks and sources, taking both specialized and the general learning into account. And this paradigm shows great capability of complexity and expansibility.
% %
% Moreover, we perform in-depth analysis of the effect of joint training diverse tasks by carrying out an experimental exploration of transfer learning across vastly different data domains, task types and methods. And our study leads to several insights and recommendations for this new diagram. 
% % 在多种多样的下游任务上做了全面的验证，点题 Universal Visual Representation，说一些优势明显的结果
% Compared to other pretraining methods, our method shows the ability of robustness and generalization to the various tasks. We benchmark our methods on the 11 transfer datasets which demonstrate remarkable gains over the representation learning methods, proving effectiveness of X-Learner for universal visual representation.



% Compared with training a network for single task, multi-task learning can not only reduce the complexity of multiple tasks (i.e. image classification, object detection) but also take advantage of the relationship between tasks during training.  Although multi-task learning can improve the feature expression ability of the backbone in a certain, using multi-task learning as pretraining is still an open problem. Thousands of labeled data are difficult to use. We explore a new pretraining paradigm of use multi-task learning that aims to make use of the complementary capabilities of datasets and tasks as effectively as possible. As far as we know, \textit{X-Learner} is the first work that uses supervised multi-task learning for representation learning. And it's highly scalable for multiple visual tasks learning. Compared to other pretraining methods, our method shows the ability of robustness and generalization to the various tasks. We benchmark our methods on the 11 transfer datasets which demonstrate stable gains over the representation learning methods. 
